A True Positives Theorem for a Static Race Detector - Extended Version

RacerD is a static race detector that has been proven to be effective in engineering practice: it has seen thousands of data races fixed by developers before reaching production, and has supported the migration of Facebook's Android app rendering infrastructure from a single-threaded to a multi-threaded architecture. We prove a True Positives Theorem stating that, under certain assumptions, an idealized theoretical version of the analysis never reports a false positive. We also provide an empirical evaluation of an implementation of this analysis, versus the original RacerD. The theorem was motivated in the first case by the desire to understand the observation from production that RacerD was providing remarkably accurate signal to developers, and then the theorem guided further analyzer design decisions. Technically, our result can be seen as saying that the analysis computes an under-approximation of an over-approximation, which is the reverse of the more usual (over of under) situation in static analysis. Until now, static analyzers that are effective in practice but unsound have often been regarded as ad hoc; in contrast, we suggest that, in the future, theorems of this variety might be generally useful in understanding, justifying and designing effective static analyses for bug catching.

==> algorithm.tex <==

\section{An Algorithm for Compositional Race Detection}
\label{sec:algorithm}

The goal of this section is to convey the key ideas of the \racerd algorithm in an informal, but comprehensive manner.
The explanation here is intended to be an ideal starting point for a reader that wishes to implement a similar approach.
By contrast, Section~\ref{sec:formalisation} formally presents the analysis algorithm and proves that it reports no false positives under certain assumptions.
Section~\ref{sec:evaluation} presents emprical evidence that this approach is effective for finding real races with a high signal-to-noise ratio.

\newcommand{\context}{mutual exclusion information~}
%\shb{I don't like the term ``context information'' because ``context'' is too overloaded. I thought about ``metadata'' too, but that's even less descriptive. Ideas?}
%\poh{All three of these things are about providing mutual exclusion}
% Brilliant! thanks Peter!

At its core, \racerd is a simple analysis that does only two things: (1) record the set of heap accesses performed by a procedure, and (2) compute \context to associate with each access.
The representation of a heap access is intentionally quite basic---we record only the syntactic \emph{access path}~\cite{Jones-al:POPL79} along with its location.
We do not try to reason about what address(es) the path might refer to or utilize a global alias analysis.
Thus, the effectiveness of the analysis depends entirely on selecting useful \context to associate with each access.
%% \tldr{Explain why we get away with such a simple heap abstraction and convince you that it's a reasonable idea}
%% At first glance, this representation might seem too coarse to form the backbone of an effective race detector.
%% Previous techniques \shb{cite Chord + others} build on a may-alias or must-alias analysis in order to determine which accesses touch the same memory.
%% But we cannot rely on a global heap analysis like this because our algorithm needs to be compositional.
%% We don't know how to efficiently analyze small code changes in a large codebase with a global analysis, and analyzing code changes is key for the effective deployment of \racerd.
%% A compositional heap analysis such as bi-abduction \shb{cite bi-abduction and maybe Dilligs} might be suitable, but the overapproximate nature of these analyses makes it difficult to achieve our goal of reporting no false positives under reasonable assumptions.
%% In addition, these analyses are much more complex than simply recording access paths.

%% We have found that access paths are actually an ideal abstraction for building an underapproximate race detector.
%% Though they seem purely syntactic, we have formulated a set of access path \emph{stability} conditions that imply must-aliasing of syntatically identical paths.
%% \shb{give intuition here, or just forward ref?}
%% These conditions are formalized in Section~\ref{sec:formalisation}, and we present empirical evidence that we can find many real races involving stable paths in Section~\ref{sec:evaluation}.


\racerd's abstract domain is a product domain consisting of four subdomains.
Three of the domains compute \context:

\begin{enumerate}
\item \textbf{Locks domain}: detects mutual exclusion due to being protected by the same lock.

\item \textbf{Threads domain}: detects mutual exclusion due to running on the same thread

\item \textbf{Ownership domain}: detects mutual exclusion owing to memory that is held exclusively my one thread, and
thus not shared between threads. This is similar to the way an thread escape analysis is used in optimization or in overapproximate race detectors~\cite{Choi-al:OOPSLA99, Naik-al:PLDI06}.

\end{enumerate}

The fourth domain maintains an assocation between each access performed by the program and its \context.
%Technically speaking, the analysis is a reduced product between the access domain and the cartestian product of the three \context domains.

%\shb{TODO: need to adjust this depending on whether we express a summary as a function or abstract state with footprint holes. Pros of the first approach: instantiation is simple, Cons: hard to explain what it means to ``aggregate'' functions. Second approach basically has opposite tradeoffs; instantiation is complicated, but aggregation makes sense. Leaning toward second}
After analyzing a procedure using \racerd's domains, the final abstract state of the procedure is converted into a \emph{summary}.
This conversion replaces program variables that are formals or return values of the current procedure with symbolic \emph{footprint} variables.
Such symbolic variables are often called `auxiliary' or `ghost' variables in Hoare logic, and are used in specifications to provide a binding for quantities (such as a location identity) that do not change during computation. Auxiliary variables provide a simple means of abstraction in forming procedure specifications, and are used in the compositional shape analysis of \cite{Calcagno-al:JACM11}
to name locations in the pre-state when forming a procedure summary; we use them for a similar purpose here.
A summary is instantiated at a call site by binding the symbolic footprint variables in the summary to their actual abstract values in the caller abstract state and joining the result with the caller abstract state.
%A \racerd summary is a function from a callee abstract state and and callee parameter indexes (including a special return index) to an abstract state.
%A summary is instantiated at its call site by applying the summary to the pre-call abstract state and using the result of the application as the post-call abstract state.
We will explain each of \racerd's domains and how they contribute to the summary in Section~\ref{sec:abstractDomains}.

After \racerd finishes computing the summaries for all of the procedures in a single class, it aggregates the accesses from each summary to determine which pairs of accesses may race.
Section~\ref{sec:reporting} describes how this process works.


%A procedure summary is a function from abstract state and parameter indexes to an abstract state.

%We will begin by explaining how we perform the first two steps for a single procedure, then show how we extend this scheme to inteprocedural analysis by creating summaries from the intraprocedural state and applying them at call sites. Finally, we will show how we put the pieces together to report races in the third step.

%% Conceptually, \racerd's algorithm for race detection consists of three steps:

%% \begin{enumerate}

%% \item \textbf{Summarize the heap accesses peformed by a procedure}

%% The analyis records the heap reads and writes directly performed by a procedure as well as the accessess in its (transitive) callees. It remembers when locks were held at the time of an access to avoid reporting on pairs of accesses that might be safe due to mutual exclusion. It also uses \emph{ownership} information to discard accesses to memory that is not shared by multiple threads (and thus cannot be involved in a race).

%% \item \textbf{Infer which procedures may run in a concurrent context}

%% By default, the analysis assumes that a procedure cannot be run concurrently with code on other threads. We use signals such as usage of locks, annotations like \code{@ThreadSafe}/\code{@GuardedBy}, and calls to \code{assertMainThread} to determine when a procedure can be used in a concurrent context and what other code can be run at the same time.

%% \item \textbf{Report races on pairs of conflicting accesses reachable from these procedures}

%% \racerd aggegrates the accesses from all of the procedures in a single file that may run in a concurrent context. It reports a race for each pair of accesses to the same memory that may conflict based on the locking and concurrent context information computed by the analysis. The analysis report a full stack trace to each access to make it possible for developers to understand complex interprocedural race reports.

%% \end{enumerate}

\subsection{\racerd abstract domains}
\label{sec:abstractDomains}

We will explain each of the three standalone \context domains first, then show how the access domain ties everything together.

\subsubsection{Locks domain: counting locks held}

\racerd focuses on identifying accesses that are unsafe because they are not guarded by any lock rather than accesses that are unsafe because they are guarded by the wrong lock(s).
Thus, \racerd's lock domain chooses to ignore lock identities--it doesn't attempt to track \emph{which} lock is being acquired or released.
Instead, it overapproximates the \emph{number} of locks held at a given program point.
This is consistent with our desire for underapproximate reporting of races; if we know that a lock may be held at the time when an access occurs, we will not report the access.

Abstract values $\lock$ in the lock domain are non-negative integers or a special $\top$ element.
The ordering on integer elements is $\leq$, and all integer values are below the $\top$ element on the ordering.
%We define join as $\hat\sigma_1 \sqcup \hat\sigma_2$ = $min(\top, max(\hat\sigma_1, \hat\sigma_2)$.
Widening any two abstract values produces the $\top$ value.
We define a liftings of integer addition (\texttt{+}$^{\top}$) and subtract (\texttt{-}$^{\top}$) to handle the $\top$ element in the obvious way (any value \texttt{+}/\texttt{-} $\top$ is also $\top$).
Acquiring a lock is modeled as incrementing the abstract value, and releasing a lock is modelled as decrementing the abstract value.

The intial lock count for a procedure is $\textbf{1}$ if the procedure is marked \code{synchronized} and $\textbf{0}$ otherwise.
If the number of locks held at the end of a procedure is $\lock_{post}$, we use $\lock_{post}$ \texttt{-}$^{\top}$ $\textbf{1}$ if the procedure is marked \code{synchronized} and $\lock_{post}$ otherwise.
%We apply summaries by adding the number of locks held in the caller to the number of locks held in the callee using \texttt{+}$^{\top}$.

\begin{wrapfigure}{l}{0.25\textwidth}
\vspace{-18pt} % please halp, if you know a less hacky way!
\begin{lstlisting}[language=java]
synchronized (lock1) {
  synchronized (lock2) {
    x.f = ...
  }
  y.g = ...
}
z.h = ...
\end{lstlisting}
\vspace{-20pt}
\end{wrapfigure}
As we will see later, the lock count is only used to determine whether a lock might be currently held during an access (i.e., we only care whether it's zero or nonzero).
Given this, a simple boolean abstraction might seem like a better choice than our counting domain.
However, a boolean abstraction does not work well in the presence of nested locks.
Consider the simple example inline.
A boolean domain will be unable to determine that a lock is held during the accesses to \code{x.f} and \code{y.g}, but not during the access to \code{z.h}.
We use a counting domain instead of a simpler boolean abstraction in order to avoid this issue.


%% Because the access occurs inside a \code{synchronized} block, \racerd also records that one lock was held at the time of the access.
%% Note that \racerd does not track the identity of the lock held (i.e., the abstract state doesn't say anything about \code{mLock}).
%% This is consistent with our desire for underapproximation.
%% Although we could track identities and then use a global may-alias analysis to determine when two locks might be the same, we would run into the same non-compositional problem described above.
%% In addition, the Facebook engineers who helped us develop \racerd told us that the most common concurrency bugs in their domain of interest involved missing locks rather than using the wrong lock.
%% We don't need to track lock identities to find these bugs.

%% Thus, \racerd's lock domain chooses to ignore lock identities and overapproximate the number of locks held at a given location.
%% We use a counting domain instead of a simpler boolean abstraction in order to avoid false alarms due to nested locks.

%% For the second access in Figure~\ref{fig:accessPathTracking}, \racerd notes that the access was a read of \code{o.g} at line 6.
%% Because this access occurs outside of the \code{synchronized} block, the number of locks held is recorded as zero.
%% \racerd records this access even though it was guarded by an `if` statement. The analysis makes no attempt to reason about the reachability of accesses and thus will record every access it encounters unless the access is \emph{owned} or \emph{unstable}, as we will now explain.

%% \begin{figure}
%% \begin{lstlisting}[language=java,style=number]
%% synchronized (mLock) {
%%   o.f = ...
%%   // { (o.f, write, 1 lock, line 3) }
%% }
%% if (*) { System.out.println(o.g); }
%% // { (o.f, write, 1 lock, line 3) , (o.g, read, 0 locks, line 5) }
%% \end{lstlisting}

%% \label{fig:accessPathTracking}
%% \end{figure}

\subsubsection{Threads domain: concurrent context inference}
\label{sec:concurrentContextInfererence}

\shb{TODO: Double duty of inference + mutual exclusion is confusing here. Focus on the mutual exclusion story}
In order for \racerd to identify races, it needs to understand which accesses can run concurrently on separate threads.
The simplest approach here would be to assume that any code fragment can be run in parallel with any other code fragment (including itself).
This would be far too noisy to be useful.
Instead, \racerd assumes that a code fragment cannot be run in parallel with \emph{any} other code unless it sees ``evidence'' that the fragment is intended to be run in a concurrent context.
The forms of evidence \racerd considers are:

\begin{itemize}
\item Usage of locks. Code should only use locks if it is meant to be run in a concurrent context!
\item Usage of \code{java.util.concurrent} annotations like \code{@ThreadSafe} or \code{@GuardedBy}. We assume that developers use these anotations to document that the annotated code is intended to be used in a concurrent context.
\item Usage of Android utility functions like \code{assertMainThread()} and \code{assertOnBackgroundThread()}. We assume these functions should only be used if there's a possibility that the code fragment can be run on a thread that's running concurrently with other threads.
\end{itemize}

\paragraph{Abstracting threads}
%\shb{TODO: say that identifying thread spawning structure in a compositional manner is hard, which is why we used this evidence-based approach. Can also contrast with the manual approach taken by tools like Chord}

\racerd's thread abstaction infers which threads may run in parallel with the thread of the current procedure.
It uses three abstract values: the current procedure runs sequentially (\texttt{NoThread}), the current procedure runs on the main thread (\texttt{AnyThreadButMain}), or the current procedure runs on a thread that can interleave with any other thread (\texttt{AnyThread}).
An access that is \texttt{NoThread} can't race with any accesses.
An access that is \texttt{AnyThreadButMain} can race with \texttt{AnyThread} accesses, but not with other \texttt{AnyThreadButMain} accesses

These abstract values form a domain with the partial order \texttt{NoThread} $\sqsubseteq$ \texttt{AnyThreadButMain} $\sqsubseteq$ \texttt{AnyThread}.
The concretization of an abstract value is a set of thread id's whose execution may interleave with the thread executing the current procedure.
Let $t_{main}$ be the thread id of the main thread.
Then we can define the concretization as follows:

\[
\gamma(t) \eqdef 
\begin{cases}
\emptyset \text{ if } t = \texttt{NoThread} \\
\{ t | t \neq t_{main} \} \text{ if } t = \texttt{AnyThreadButMain} \\
2^t \text{ if } t = \texttt{AnyThread}
\end{cases}
\]
The default abstract value for a procedure is \texttt{NoThread}.
This prevents us from reporting false positives on code that is only run in a sequential context.

Annotating a procedure \code{@UiThread} or calling a utility method like \code{assertMainThread} changes the abstract value to \texttt{AnyThreadButMain}.
This allows us to capture some common safety patterns used in Android programming.
In Android applications, important tasks typically run either on the main (UI) thread, or on a ``background'' worker thread that can run in parallel with the main thread.
Code that runs on the main thread can run in parallel with code running on background threads, but not with itself.
Code that runs on background threads can typically run in parallel with everything, including multiple copies of the same code.
Developers leverage the restricted nature of the main thread to use fewer locks: code that would be vulnerable to self-races when run on a background thread does not need to be protected when it can only run on the main thread.
\racerd reported many spurious races on the main thread before we enhanced its abstraction of threads to understand this pattern.

Finally, annotating a procedure \code{@ThreadSafe}, tagging it with the \code{synchronized} keyword, or using a lock in the body of a method (e.g., a \code{synchronized} block or lock object like \code{java.util.concurrent.Lock.lock()}) changes the abstract value to \texttt{AnyThread}.
Annotating a class \code{@ThreadSafe} is the same as annotating all of its non-\code{private} methods as \code{@ThreadSafe}.
Subtypes of the annotated class are treated in the same way.
Thus, our interpretation of a \code{@ThreadSafe} class $C$ is: ``Any non-\code{private} method $m$ of $C$ can be safely called in parallel with all other non-\code{private} methods of $C$ and its subclasses, including $m$ itself.''
We have found that this generally fits well with the intention developers have when marking a class \code{@ThreadSafe}: it's impossible for a client of the class to use it in a way that causes a race.
%Using a \code{synchronized} block or lock object (e.g., \code{java.util.concurrent.Lock.lock()}) in the body of a method changes the abstract value to \code{AnyCode} if the current abstract value is \texttt{NoCode} and leaves the abstract value unchanged otherwise.
% SHB: assuming this ^ isn't worht taking the time to explain

%\paragraph{Limitations}

%\shb{Comment on lessons from D6193062--inferring concurrent context from starting new threads seems natural, but leads to an unacceptable number of false positives due to task queues that can run on the same thread. In essence, violates the assumption that everything can run in parallel}

\subsubsection{Ownership domain: identifying clearly safe accesses}
\shb{TODO: make it clear that this is involved in the implementation but not the formalism. Explain relationship to wobbly paths}

An individual access may be involved in a race if it can run concurrently with another accesses to the same memory.
Clearly, tracking every syntactic access path yields an overapproximation of the accesses that may be involved in a race.
Since our goal is high-confidence bugfinding rather than verification, we would like to shrink this set by pruning away accesses that \emph{may} not be involved in a race.
\racerd uses an ownership analysis to for this purpose.

Intuitively, an owned access path should hold a value that has not leaked to another thread.
\racerd computes a \emph{may}-ownership analysis that overapproximates the set of owned access paths at each program point.
It leverages the fact that an access path holding freshly allocated memory is owned and aggressively propagates ownership across assignments.

The ownership abstract domain maps access paths to ownership abstract values, which are abstractions of concrete addresses.
The two different abstract values used to represent ownership states are $\unowned$ and $\ownedif{n_1, \ldots, n_i }$.
An $\unowned$ value is potentially unsafe to access; intuitively, it represents an address that may be reachable from local variables of multiple threads
$\mathsf{OwnedIf}$ represents ownership that is conditional on ownership of \emph{all} of the formal parameters at the given indexes.
An abstract value like $\ownedif{\{1, 2\}}$ value is owned \emph{if} both the first and second formal parameter are owned at the call site of the current procedure.
$\ownedif{\emptyset}$ means that the value is owned.

The $\mathsf{OwnedIf}$ values form a powerset lattice with $\ownedif{\emptyset}$ as the bottom element.
The $\unowned$ value is used as a distinguished top value for the powerset lattice.

Initially, each local and global variable is mapped to $\unowned$, and the $i$th formal parameter is bound to $\ownedif{ \{i\} }$.
Assignment to an access path propagates the ownership value bound to the righthand side of the assignment to the lefthand side of the assignment.


%% \begin{figure}
%% \begin{lstlisting}[language=java,style=number]
%% Obj o1 = new Obj();
%% // accesses: {}, owned: { o1 }
%% o1.f = ... // direct access to owned path--safe
%% o1.f.g = ... // access rooted in owned path -- assume safe
%% Obj o2 = o1; // propagate ownership to o2
%% // accesses: {}, owned: { o1, o2 }
%% o2.f = ... // o2 owned, safe
%% sGlobal = new Obj(); // ownership not propagated to gobal
%% // accesses: {}, owned: { o1, o2 }
%% sGlobal.h = ... // global access; not owned
%% // accesses: { (sGlobal.h, 0 locks, line 2) }, owned: { o1, o2 }
%% o1 = sGlobal; // o1 no longer owned
%% // accesses: { (sGlobal.h, 0 locks, line 2) }, owned: { o2 }
%% \end{lstlisting}

%% \label{fig:basicOwnership}
%% \end{figure}

%% Figure \ref{fig:basicOwnership} demonstrates \racerd uses ownership to discard
%% \code{o1} is initially marked as owned because it is bound to a freshly constructed object.
%% This allows \racerd to avoid tracking both direct (\code{o1.f}) and indirect (\code{o1.f.g}) accesses to paths rooted in \code{o1}--it assumes these accesses are safe because they are roooted in an owned path.

%% When \code{o2} is initialized to \code{o1}, \racerd propagates the ownership of \code{o1} to \code{o2}, and accesses rooted in \code{o2} are also assumed to be safe.
%% By contrast, accesses rooted in the global variable \code{sGlobal} are never treated as safe even when \code{sGlobal} is directly assigned to a freshly allocated object.
%% Because \code{sGlobal} is not a local variable, the freshly allocated value may be readable/writable by other threads.
%% Thus, \racerd chooses to track the access to \code{sGlobal.h} despite the assignment to a fresh object on the previous line..

%% If we reassign the local `o1` to `sGlobal`, \racerd will no longer consider `o1` to be owned.
%% This means that subsequent accesses to `o1` will be tracked.

%% \shb{these rules are quite straightforward to apply locally, but they really shine in eliminating false positives in interprocedural analysis}

%\paragraph{Using ownership}

%Note that the set of accesses after ownership pruning is neither an underapproximation nor an underapproximation of the accesses that may be involved in a race.
%The initial set of accesses is overapproximate, but because we prune this set using a \emph{may}-ownership analysis, we throw away accesses that could be involved in a race.
%But this is not an underapproximation either; unowned/stable accesses need not be involved in a race.
%The technique we use to aggregate and match conflicting accesses (Section ~\ref{sec:reporting}) is what actually ensures that we report an underapproximation of the possible races.

\subsubsection{Access domain: putting it all together}

The access domain captures a snapshot of the relevant state at the time of each syntactic access.
It records the heap reads and writes directly performed by a procedure as well as the accessess in its (transitive) callees.
Abstract values in the access domain are $\angled{\text{access path}, \textsf{Read}/\textsf{Write}, \text{location}}$ 3-tuples.
%\shb{TODO: explain container accesses too, if we have space}
For example, the code \code{x.f.y = 2;} at location $l$ would generate the abstract values (\code{x}, \textsf{Read}, $\ell$), (\code{x.f}, \textsf{Read}, $l$), and (\code{x.f.y}, \textsf{Write}, $l$).
Each abstract value is associated with \context tracked by the other three domains.
The domain itself is a powerset of access-\context pairs.

%from these abstract values to \context (i.e., an abstract value from the product domain of the to-be-described locks, threads, and ownership domains)\footnote{For efficency reasons, we actually implement the domain as a mapping from \context to accesses, since many accesses tend to share the same context. We explain the reverse mapping above for ease of exposition}.


%This domain is overapproximate in the sense that it genuinely captures every possible heap access in the program.
%But as we will see in Section~\ref{sec:reporting}, this still supports our aim of underapproximation in that our concretization of an access path is very underapproximate---two access path concretize to the same address if and only if they are syntactically equal.
%\shb{This is the only domain that's overapproximate, at least in the sense that it genuinely overapproximates the set of syntatic access paths. However, our concretization is very underapproximate==two access paths concretize to the same address iff they are syntactically equal.}

\paragraph{Applying procedure summaries}

\begin{figure}

\[
apply(\lock_{caller}, \lock_{callee}) \eqdef \lock_{caller} +^{\top} \lock_{callee}
\]

\[
apply(t_{caller}, t_{callee}) \eqdef 
\begin{cases}
\textsf{AnyThreadButMain} \text{ if } t_{callee} = \textsf{AnyThreadButMain} \\
t_{caller} \text { otherwise }
\end{cases}
\]

\[
O(\e) \eqdef 
\begin{cases}
o \text{ if } \e = \pi \wedge (\pi, o) \in O \\
\unowned \text{ if } \e = \pi \wedge \pi \notin dom(O) \\
\ownedif{\emptyset} \text{ otherwise }
\end{cases}
\]


\[
apply(O_{caller}, o_{callee}, \vec{\e}) \eqdef 
\begin{cases}
\unowned \text{ if } o_{callee} = \unowned \\
\ownedif{\emptyset} \text { if } o_{callee} = \ownedif{\emptyset} \\
\bigsqcup\limits_{i \in I} O_{caller}(\e_i) \text{ if } o_{callee} = \ownedif{I}
\end{cases}
\]

\[
apply(O_{caller}, O_{callee}, \vec{\e}, \texttt{ret}) \eqdef
O_{caller}[\texttt{ret} \mapsto apply(O_{caller}, O_{callee}(ret), \vec{\e})]
\]

% formatting crimes against humanity follow; read at your own risk
\begin{align*}
& apply(A_{caller}, A_{callee}, \vec{\e}) \eqdef A_{caller} ~\sqcup~ \\
& \hspace{10pt} \{ \angled{c, apply(\lock_{caller}, \lock), apply(t_{caller}, t), apply(O_{caller}, o, \vec{e})} ~|~ \angled{c, \lock, t, o} \in A_{callee} \}
\end{align*}

\begin{align*}
& apply(\angled{\lock_{caller}, t_{caller}, O_{caller}, A_{caller}}, \vec{\e}, \texttt{ret}, \\
& \hspace{25pt} \angled{\lock_{callee}, t_{callee}, O_{callee}, A_{callee}}) \eqdef \\
& \hspace{10pt} \text{let } \lock' = apply(\lock_{caller}, \lock_{callee}) \text{ in} \\
& \hspace{10pt} \text{let } t' = apply(t_{caller}, t_{callee}) \text{ in} \\
& \hspace{10pt} \text{let } O' = apply(O_{caller}, O_{callee}, \vec{\e}, \texttt{ret}) \text{ in} \\
& \hspace{10pt} \text{let } A' = apply(A_{caller}, A_{callee}, \vec{\e}) \text{ in} \\
& \hspace{10pt} \angled{\lock', t', O', A'}
\end{align*}

\caption{Applying summaries.}

\label{fig:summaries}
\end{figure}

An abstract state in our analysis is a four-tuple: $\angled{l, t, O, A}$: lock count $l$, thread $t$, access path-ownership map $O$, and set of access snapshots $A$.
As we have explained, the first three domains track the current \context and the access snapshots $A$ associate the heap accesses performed so far with \context at the time of each access.

A summary has the same type as an abstract state.
At a high level, applying a summary to an abstract state at a call site involves two steps:
\begin{enumerate}
\item Updating the caller's \context based on the locks acquired, threading information, and ownership value returned by the callee.
%For example, if a lock is acquired and not released in the callee
\item Updating the callee's access snapshots with the caller's \context, then joining the updated snapshot set with the caller's access snapshots. 
%For example, if a lock is held in the caller, then the lock count associated with each access in the callee should be bumped by one.
\end{enumerate}

Figure~\ref{fig:summaries} defines an $apply$ function for combining caller and callee state for each of four components of our abstract state.
We will walk through each one and explain how it works with examples.

\paragraph{Summarizing callee locks}
The $apply(\lock_{caller}, \lock_{callee})$ function for the locks domain adds the number of locks held in the caller $\lock_{caller}$ to the number of locks held in the callee $\lock_{callee}$ using the lifted addition operator \texttt{+}$^{\top}$.
This makes sense because we wish to overapproximate the number of locks held after the call, and the sum of the current lock count and the number of locks acquired in the callee will achieve this.
In practice, $\lock_{callee}$ will typically be $\textbf{O}$ unless the callee acquires a lock without releasing it (e.g., \code{void acquire() \{ mLock.lock(); \}}.

\shb{TODO: rework this after simplifying the discussion of the threads domain}

\paragraph{Summarizing callee threads}
%\shb{TODO: after writing all of this, I'm less sure that it's interesting/important. Also, some improvments are evident: if a callee is \texttt{AnyThread} *and* acquires a lock and the caller is \texttt{oThread}, we should get \texttt{AnyThread} (would help fix the immutable problem). Additionall, should have an abstract value for ``background thread'' that's distinct from \texttt{AnyThread} and \texttt{AnyThreadButMain}}

If a caller runs in a concurrent context, then clearly its callees do too.
However, consider the case when we have evidence that a callee is expected to run in a concurrent context, but don't know anything about what context is expected for the caller.
Inheriting the callee's context (i.e., joining the abstract values of the caller and callee) seems like a natural choice.
However, we found that this introduces a large number of false positives in practice.
The primary problem is this: calling code that is safe to run in a concurrent context does not necessarily imply that the caller will run in a concurrent context.

To see why this is true, consider the example in Figure~\ref{fig:immutableThreadSafe}. 
The problem captured in this example is that in practice, \code{@ThreadSafe} is sometimes intended to mean only ``safe to use in a concurrent context'' (e.g., immutable classes) and sometimes intended to mean ``safe \textbf{and} intended to be used only in a concurrent context'' (e.g., a thread-safe data structure like \code{ConcurrentHashMap}).
\racerd does not have a reliable way of understanding which meaning is intended.

\begin{figure}
\begin{lstlisting}[language=java,style=number]
@ThreadSafe class ImmutableData {
  private final int mData;
  public ImmutableData(int data) { this.mData = data; }
  int getData() { return mData; }
}

public void sequential(ImmutableData data) {
  this.mField = data.getData();
}
\end{lstlisting}

\caption{Developers often annotate immutable classes like \code{ImmutableData} with \code{@ThreadSafe}. \code{ImmutableData} can be safely used in either a sequential or concurrent context, but class that uses \code{ImmutableData} may or may not be run in a concurrent context. If we assume that the \code{sequential} method runs in a concurrent context because it uses the \code{getData} method of a \code{@ThreadSafe} class, it will lead us to (incorrectly) report a self-race on the write to \code{this.mField}.}

\label{fig:immutableThreadSafe}
\end{figure}

To handle this, $apply(t_{caller}, t_{callee})$ chooses to use \texttt{AnyThreadButMain} as the state after the call if the callee's abstract value is \texttt{AnyThreadButMain} and the caller's abstract value otherwise.
The idea is that if a callee is known to run on the main thread (e.g., it calls \code{assertMainThread}), then the caller must also run on the main thread.
But in any other case, the callee's context doesn't necessarily tell us anything about the caller's context.

\paragraph{Summarizing callee ownership}

%% \begin{figure}
%% \begin{lstlisting}[language=java,style=number]
%% static Builder make() { return new Builder(); }
%% // summary: ret |-> Owned

%% Builder setX(int x) { 
%%   // this |-> OwnedIf({0})
%%   this.x = x;
%%   return this; 
%% } // summary: this |-> OwnedIf({0}),  <this.x, Write, OwnedIf({0})>

%% Builder useBuilder() {
%%   Builder b1 = make();
%%   // b1 |-> Owned
%%   Builder b2 = b1.setX(1); // b1 is bound to formal 0
%%   // b1 |-> Owned, b2 |-> Owned <this.x, Write, Owned>
%%   return b2;
%% } // summary: ret |-> Owned
%% \end{lstlisting}

%% \caption{Example of the commonly used \code{Builder} pattern in Java. \racerd's propagates ownership information interprocedurally Understanding that all three procedures return ownership and that no accesses in this example can be}

%% \label{fig:interprocOwnership}
%% \end{figure}

\begin{figure}
\begin{lstlisting}[language=java,style=number]
static Builder make() { return new Builder(); }
// summary: ret |-> Owned

Builder setX(int x) {
  ...
  return this;
} // summary : ret |-> OwnedIf({this})

Builder useBuilder() {
  Builder b1 = make();
  // b1 |-> Owned
  Builder b2 = b1.setX(1); // b1 is bound to callee formal this
  // b1 |-> Owned, b2 |-> OwnedIf({b2})
  // b1 |-> Owned, b2 |-> Owned
  return b2;
} // summary: ret |-> Owned
\end{lstlisting}

\caption{Example of the commonly used \code{Builder} pattern in Java. \racerd propagates ownership information interprocedurally to understand that all three procedures return ownership.}

\label{fig:interprocOwnership}
\end{figure}


The utility function $O(e)$ uses the access path to ownership value mapping to determine whether $e$ is owned or not.


%that takes the caller abstract state, the callee abstract state, and the actual expressions $\vec{\e}$/return value \texttt{ret} at the call site as input and returns a new abstract state that reflects the effects of the call.


A%pplying a summary to an abstract state at a call site involves replacing the footprint variables in the callee summary with their values in the caller


\subsection{Reporting Errors}
\label{sec:reporting}

\shb{TODO: better transition}
We will now explain how \racerd uses the procedure summaries it computes in order to report potential races.

\paragraph{Aggregating summaries}

Once \racerd has finished analyzing each procedure in a class, it aggregates the summaries from all of the procedures to group accesses that might be to the same memory.
A summary is essentially a set of (access path, access kind, access location, locks, thread) tuples representing accesses to unowned memory.
The aggregation step creates a map from an access path name to a set of tuples that share the same syntactic access path.
If the access path is \textbf{stable} in the sense explained in Section~\ref{sec:formalisation}, every access in the set touches the same memory.
If we wished to trade off more warnings for a higher risk of false positives, we could used a more relaxed notion of access path equality (e.g., assume that access paths ending in the same field or with the same type may touch the same memory).

\paragraph{Matching accesses}

After aggregating all of the tuples that touch the same syntactic access path, \racerd attempts to find racy accesses by considering each pair of distinct access tuples.
Two accesses to the same stable syntactic path do not necessarily race.
A potential data race between a pair of accesses can be prevented if a lock during each access, if the accesses occur on threads that cannot run in parallel, or if neither of the accesses is a write.

\racerd reports a pair of accesses as read/write race if all of the following conditions hold:
\begin{enumerate}
\item \emph{Kinds}: $kind(a_1)$ = \texttt{Write} $\vee$ $kind(a_2)$ = \texttt{Write} (at least one of the accesses is a write).
\item \emph{Locks}: $lock(a_1) = 0$ $\vee$ $lock(a_2) = 0$ (at least one of the accesses is not protected by a lock).
\item \emph{Threads}: $thread(a_1) \sqcap thread(a_2) \neq \texttt{NoThread} \wedge thread(a_1) \sqcup thread(a_2) = \texttt{AnyThread}$  (both accesses occur in a concurrent context, and at least one occurs off of the main thread).
\end{enumerate}

In addition, \racerd reports an individual access $a$ as a write/write race if $kind(a)$ = \texttt{Write}, $lock(a)$ = 0, and $thread(a)$ = \texttt{AnyThread} (i.e., the access is a write not protected by a lock that can run in parallel with another thread running the same code).

\subsubsection{Unrolling summaries to create interprocedural stack traces}
\shb{Talk about ``last callee'' trick that makes storing full stack traces constant in trace depth instead of quadratic}


==> chord-table.tex <==

\begin{table}[t]
  \centering
{\small{
%\vspace{-5pt}
  \begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Program}}
    & \multirow{2}{*}{\#~Files}
    & \multirow{2}{*}{\#~LOC}
    & \multicolumn{2}{c|}{\chord}
    & \multicolumn{3}{c|}{\racerd}
    & Alarm
    %
    \\\cline{4-8}
    & & & {\scriptsize{\# Alarms}} & {\scriptsize{Runtime}} &
    {\scriptsize{\# Alarms}} &
                                                                      {\scriptsize{\# Unstable}} & {\scriptsize{~Runtime}}
    & Overlap
    \\\hline\hline
%
\pname{hedc} & 133 & 11,767 & 152 & 4m 47s
    & 49 & 2 (4\%) & 1.5s & 11\%
\\
\pname{ftp} & 140 & 12,050 & 522 & 5m 14s
    & 39 & 4 (10\%) & 1.5s & 20\%
\\
\pname{weblech} & 12 & 1,309 & 30 & 11m 02s
      & 9 & 0 (0\%) & 0.6s & 63\%
\\
\pname{jspider} & 214 & 7,413 & 257 & 1m 54s
      & 13 & 0 (0\%) & 1.4s & 10\%
\\
% [2pt]
% \hline
\pname{avrora} & 470 & 68,864 & 966 & 8m 49s
      & 81 & 6 (7\%)  & 7s & 18\%
\\
\pname{luindex} & 331 & 36,151 & 940 & 3m 26s
      & 183 & 5 (3\%) & 5s & 64\%
\\
\pname{sunflow} & 170 & 21,960 & 958 &  42m 44s
      & 43 & 3 (7\%) & 2.8s & 49\%
\\
\pname{xalan} & 975 & 175,784 & 1870 & 1h 47m
      & 421 & 49 (12\%) & 21.5s & 38\%
\\
\hline
  \end{tabular}
}}
%\vspace{5pt}
\caption{\racerd reports >3X fewer alarms than \chord on every benchmark, and an order of magnitude fewer alarms on four of the benchmarks. \racerd is at one or two orders of magnitude faster on all benchmarks. The ``Unstable'' column gives the number/percentage of \racerd alarms that may be false positives due to an unstable access path (see Section~\ref{sec:formalisation}). The ``Alarm Overlap'' column indicates the percentage of racy lines implicated by \chord that \emph{also} appeared in a report from \racerd.}
\label{tab:chord}
\end{table}


%% \begin{table}[t]
%%   \centering
%% {\small{
%% %\vspace{-5pt}
%%   \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
%% \hline
%% \multicolumn{1}{c|}{\multirow{2}{*}{Program}}
%%     & \multirow{2}{*}{\#~Files}
%%     & \multirow{2}{*}{\#~LOC}
%%     & \multicolumn{2}{c|}{\chord}
%%     & \multicolumn{4}{c|}{\racerd}
%%     & \multirow{2}{*}{Overlap}
%%     %
%%     \\\cline{4-9}
%%     & & & {\scriptsize{\# Alarms}} & {\scriptsize{Runtime}} &
%%     {\scriptsize{\# Alarms (R)}} & {\scriptsize{\# Alarms (F)}} &
%%                                                                       {\scriptsize{\# Unstable}} & {\scriptsize{~Runtime}}
%%     &
%%     \\\hline\hline
%% %
%% \pname{hedc} & 133 & 11,767 & 152 & 4m 47s
%%     & 82 & 49 & 2 (4\%) & 1.5s & 16
%% \\
%% \pname{ftp} & 140 & 12,050 & 522 & 5m 14s
%%     & 57 & 39 & 4 (10\%) & 1.5s & 106
%% \\
%% \pname{weblech} & 12 & 1,309 & 30 & 11m 02s
%%       & 22 & 9 & 0 (0\%) & 0.6s & 19
%% \\
%% \pname{jspider} & 214 & 7,413 & 257 & 1m 54s
%%       & 25 & 13 & 0 (0\%) & 1.4s & 25
%% \\
%% % [2pt]
%% % \hline
%% \pname{avrora} & 470 & 68,864 & 966 & 8m 49s
%%       &  365 & 81 & 6 (7\%)  & 7s & 177
%% \\
%% \pname{luindex} & 331 & 36,151 & 940 & 3m 26s
%%       & 428 & 183 & 5 (3\%) & 5s & 598
%% \\
%% \pname{sunflow} & 170 & 21,960 & 958 &  42m 44s
%%       & 236 & 43 & 3 (7\%) & 2.8s & 466
%% \\
%% \pname{xalan} & 975 & 175,784 & 1870 & 1h 47m
%%       &  2171 & 421 & 49 (12\%) & 21.5s & 712
%% \\
%% \hline
%%   \end{tabular}
%% }}
%% %\vspace{5pt}
%% \caption{Comparison of \chord and \racerd. Alarms by
%%   \racerd are given for raw (R) and filtered (F) output.}
%% \label{tab:chord}
%% \end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% The following one with +/-1 fluctuations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}[t]
%   \centering
% {\small{
% %\vspace{-5pt}
%   \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
% \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{Program}}
%     & \multirow{2}{*}{\#~Files}
%     & \multirow{2}{*}{\#~LOC}
%     & \multicolumn{2}{c|}{\chord}
%     & \multicolumn{4}{c|}{\racerd}
%     & \multirow{2}{*}{Overlap}
%     %
%     \\\cline{4-9}
%     & & & {\scriptsize{\# Alarms}} & {\scriptsize{Runtime}} &
%     {\scriptsize{\# Alarms (R)}} & {\scriptsize{\# Alarms (F)}} &
%                                                                       {\scriptsize{\# Unstable}} & {\scriptsize{~Runtime}}
%     &
%     \\\hline\hline
% %
% \pname{hedc} & 133 & 11,767 & 152 & 4m 47s
%     & 82 & 49 & 2 (4\%) & 1.5s & 28
% \\
% \pname{ftp} & 140 & 12,050 & 522 & 5m 14s
%     & 57 & 39 & 4 (10\%) & 1.5s & 110
% \\
% \pname{weblech} & 12 & 1,309 & 30 & 11m 02s
%       & 22 & 9 & 0 (0\%) & 0.6s & 19
% \\
% \pname{jspider} & 214 & 7,413 & 257 & 1m 54s
%       & 25 & 13 & 0 (0\%) & 1.4s & 30
% \\
% % [2pt]
% % \hline
% \pname{avrora} & 470 & 68,864 & 966 & 8m 49s
%       &  365 & 81 & 6 (7\%)  & 7s & 204
% \\
% \pname{luindex} & 331 & 36,151 & 940 & 3m 26s
%       & 428 & 183 & 5 (3\%) & 5s & 724
% \\
% \pname{sunflow} & 170 & 21,960 & 958 &  42m 44s
%       & 236 & 43 & 3 (7\%) & 2.8s & 524
% \\
% \pname{xalan} & 975 & 175,784 & 1870 & 1h 47m
%       &  2171 & 421 & 49 (12\%) & 21.5s & 751
% \\
% \hline
%   \end{tabular}
% }}
% %\vspace{5pt}
% \caption{Comparison of \chord and \racerd. Alarms by
%   \racerd are given for raw (R) and filtered (F) output.}
% \label{tab:chord}
% \end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% \begin{table}[t]
%   \centering
% {\small{
% %\vspace{-5pt}
%   \begin{tabular}{l|c|c|c|c|c|c@{\ }|@{\ }c@{\ }|c@{\ }|@{\ }c}
% \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{Program}}
%     & \multirow{2}{*}{\#~Files}
%     & \multirow{2}{*}{\#~LOC}
%     & \multicolumn{3}{c|}{\chord}
%     & \multicolumn{4}{c}{\racerd}
%     %
%     \\\cline{4-10}
%     & & & {\scriptsize{\# Alarms}} & {\scriptsize{\# Bugs}} & {\scriptsize{Runtime}} &
%     {\scriptsize{\# Alarms (F)}} & {\scriptsize{\# Alarms (R)}} & {\scriptsize{\# Unstable}} & {\scriptsize{~Runtime}}
%     \\\hline\hline
% %
% \pname{hedc} & 133 & 11,767 & 152 & 12 & 4m 47s
%     & 49 & 82 & 2 (4\%) & 1.5s
% \\
% \pname{ftp} & 140 & 12,050 & 522 & 75 & 5m 14s
%     & 39 & 57 & 4 (10\%) & 1.5s
% \\
% \pname{weblech} & 12 & 1,309 & 30 & 6 & 11m 02s
%       & 9 & 22 & 0 (0\%) & 0.6s
% \\
% \pname{jspider} & 214 & 7,413 & 257 & 9 & 1m 54s
%       & 13 & 25 & 0 (0\%) & 1.4s
% \\
% % [2pt]
% % \hline
% \pname{avrora} & 470 & 68,864 & 966 & 29 & 8m 49s
%       &  81 & 365 & 6 (7\%)  & 7s
% \\
% \pname{luindex} & 331 & 36,151 & 940 & 2 & 3m 26s
%       & 183 & 428 & 5 (3\%) & 5s
% \\
% \pname{sunflow} & 170 & 21,960 & 958 & 176 &  42m 44s
%       & 43 & 236 & 3 (7\%) & 2.8s
% \\
% \pname{xalan} & 975 & 175,784 & 1870 & 75 & 1h 47m
%       &  421 & 2171 & 49 (12\%) & 21.5s
% \\
% \hline
%   \end{tabular}
% }}
% %\vspace{5pt}
% \caption{Comparison of \chord and \racerd. Alarms by
%   \racerd are given for filtered (F) and raw (R) output.}
% \label{tab:chord}
% \end{table}


==> dracer-table.tex <==
\begin{wraptable}{r}{0.62\textwidth}
%\setlength{\belowcaptionskip}{-10pt}
  \centering
{\small{
\vspace{-5pt}
  \begin{tabular}{l|c|c|c|c|c}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Program}}
    & \multirow{2}{*}{\#~Files}
    & \multirow{2}{*}{\#~LOC}
    & \multicolumn{2}{c|}{\# Alarms}                      
    & {\racerd}
%
    \\\cline{4-5}
    & & &\scriptsize{\dracer} & \scriptsize{\racerd} & Runtime
    \\\hline\hline
%
\pname{SGTPuzzles}
    & 33 & 9,459 & 11 (10) & 18$^{*}$ & 12s  
%
\\
%
\textsf{OpenSudoku} & 62 & 9,021 & 1 & 14 &14s
%
\\
%
\pname{K-9 mail} & 330 & 78,503 & 2 & 185 & 2m 33s
\\
\hline
  \end{tabular}
}}
\vspace{-5pt}
\caption{Comparison of \dracer and \racerd: benchmark characteristics, detected data races and \racerd runtime.}
\label{tab:eracer}
\end{wraptable}


==> eracer-table.tex <==
\begin{figure}
  \centering
  %\vspace{-12pt}
{\small{
\vspace{-5pt}
  \begin{tabular}{l|c|c|c|c|c}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Program}}
    & \multirow{2}{*}{\#~Files}
    & \multirow{2}{*}{\#~LOC}
    & \multicolumn{2}{c|}{\# Alarms (bugs)}
    & {\racerd}
%
    \\\cline{4-5}
    & & &\scriptsize{\eracer} & \scriptsize{\racerd} & Runtime
    \\\hline\hline
%
    \pname{Duckduckgo}
    & 89 & 11,127 & 1 (1) & 5$^{*}$ (5) & 15s
%
\\
%
\textsf{Connectbot} & 122 & 47,108 & 0 (0) & 117 (>0) & 1m 38s
%
\\
%
\pname{K-9 mail} & 272 & 60,955 & 0 (0) & 138 (>0) & 2m 4s
\\
\hline
    & & &\scriptsize{\dracer} & \scriptsize{\racerd} &
    \\\hline\hline
%
\pname{SGTPuzzles}
    & 33 & 9,459 & 11 (10) & 18$^{*}$ & 12s
%
\\
%
\textsf{OpenSudoku} & 62 & 9,021 & 1 & 14 &14s
%
\\
%
\pname{K-9 mail} & 330 & 78,503 & 2 & 185 & 2m 33s
  \end{tabular}
}}
\vspace{-5pt}
\caption{ Comparison of \eracer and \racerd. The ``\# Alarms'' column gives the number of reports for each tool and a lower bound for the number of true positives in parentheses. Benchmarks for which we manually added \code{@ThreadSafe} annotations for \racerd's benefit are marked with a *.}
\label{tab:eracer}
\end{figure}

%% \begin{wraptable}{r}{0.62\textwidth}
%%   \centering
%%   %\vspace{-12pt}
%% {\small{
%% \vspace{-5pt}
%%   \begin{tabular}{l|c|c|c|c|c}
%% \hline
%% \multicolumn{1}{c|}{\multirow{2}{*}{Program}}
%%     & \multirow{2}{*}{\#~Files}
%%     & \multirow{2}{*}{\#~LOC}
%%     & \multicolumn{2}{c|}{\# Alarms}
%%     & {\racerd}
%% %
%%     \\\cline{4-5}
%%     & & &\scriptsize{\eracer} & \scriptsize{\racerd} & Runtime
%%     \\\hline\hline
%% %
%%     \pname{Duckduckgo}
%%     & 89 & 11,127 & 1 & 5$^{*}$ & 15s
%% %
%% \\
%% %
%% \textsf{Connectbot} & 122 & 47,108 & 0 & 117 & 1m 38s
%% %
%% \\
%% %
%% \pname{K-9 mail} & 272 & 60,955 & 0 & 138 & 2m 4s
%% \\
%% \hline
%%   \end{tabular}
%% }}
%% \vspace{-5pt}
%% \caption{ Comparison of \eracer and \racerd: benchmark
%%   characteristics, detected data races and \racerd runtime.}
%% \label{tab:eracer}
%% \end{wraptable}


==> impact.tex <==
\section{Industrial Deployment and Impact}

This section describes the deployment of \racerd at Facebook and its impact, particularly to the introduction of multi-threading into the Facebook Android App.

\subsection{Implementation and Deployment}

RacerD is implemented as a specialized program analysis using the Infer.AI analysis framework. The framework provides an API to Infer's backend compositional analysis infrastructure, based on abstract interpretation. You describe an ?abstract domain,? symbolic values for the analysis to track, a way to transform these values by program statements, and a way to make a specification or ?summary? of a procedure that independent of its program parts. Given this, out pops a program analysis that works compositionally and can (often) scale to big code.

\racerd is used at Facebook in both a batch-mode deployment and as a bot participating in code review. In the batch deployment developers, often ones specifically interested in catching thread safety errors before placing code into a concurrent context, run RacerD on a class and resolve as many warnings as possible. In the deployment for code review Infer runs as part of the Facebook continuous integration (CI) system. For each code change a developer submits, the CI runs Infer alongside other jobs for compilation and testing. This deployment applies to all Android developers, whether they are thinking about concurrency or not, and is aimed at catching threading regressions: Infer only reports bugs that were introduced by each code change.

Typically, a small set of expert concurrent programmers use \racerd in the batch mode, such as while they are migrating code from a sequential to a multi-threaded context. The CI deployment is then used to help prevent application programmers, who are expert in front-end features but maybe not concurrency, from introducing future regressions due to concurrency.

All told, hundreds of classes have been checked in the batch mode deployment, and over 2,000 analyzer issues have been addressed in batch and CI combined (with the majority being CI) in the past X months. The issues addressed divide between non-functional changes where annotations are added that document threading assumptions and functional changes that avoid races, with each category having seen fixes numbering in the hundreds.

In order for Infer to be effective as part of the CI, the analysis must report issues quickly and use resources efficiently. We have found compositional analysis essential for meeting these requirements. With a whole-program analysis, the only obvious way to analyze a code change is to reanalyze the entire app. On a machine much more powerful than the ones used in the CI, running Infer on the Facebook Android app takes about 130 minutes. On code changes, Infer can run much faster. The graph below shows the distribution of Infer running times on a code changes over a one week period.


PUT DIAGRAM OF WEEKLY RUNTIMES

\subsection{Application to UI Components}


A toy litho program with a phabricator bug report. Must be interprocedural. Include a diagram of a bit of a tree.

How classes were checked before going multi-threaded. Typical workflow for multi-threading experts.

Something about annotations.

Something about 5 percent perf win an how important that was.

Something about moving engagement+revenue (the solicitors can make us remove it if they don't like it.) Maybe we can even slip in a vague statement.

\begin{quote}
Thus, \racerd has directly enabled a project that moved metrics related to performance, engagement and revenue.
Usually, arguments for the value of static analysis revolve around internal technical issues of code quality.
This is one of the few times  (in fact, the only time) we are aware of that static analysis has been directly implicated in moving core global metrics at a major company.
\end{quote}




==> limitations.tex <==
\section{Limitations}
\label{sec:limitations}

\is{Tell what learned \wrt structuring the semantics of the analysis.}

\is{Tell how different from what is described in the previous paper.}

Our completeness result is carried out in the presence of the
following assumptions, which are the limitations of the approach and
are left for the future work to address.

\begin{itemize}
\item No recursion -- only stratified call hierarchies;

\item No aliasing between initial class fields;

\item Deep ownership hypothesis;

\item A single lock;

\end{itemize}



==> outline.tex <==
\section*{Proposed Outline}
\label{sec:proposed-outline}


\subsection*{What we have now}
\label{sec:what-we-have}

\subsection*{What we are aiming for}
\label{sec:what-we-have}


\subsection*{TODO}

\begin{itemize}

\item Hello-world example on the ideas with something like
  pre-stability (Java in the presence of reflection?). Something that
  is screwed in the presence of extensive aliasing, \eg, escape analysis?

\item Switching off the ownership.

\item Tweaks in stability detection. 

\end{itemize}

